"You Are An Expert Linguistic Annotator": Limits of LLMs as Analyzers of Abstract Meaning Representation

Large language models (LLMs) show amazing proficiency and fluency in the use of language. Does this mean that they have also acquired insightful linguistic knowledge about the language, to an extent that they can serve as an "expert linguistic annotator"? In this paper, we examine the successes and limitations of the GPT-3, ChatGPT, and GPT-4 models in analysis of sentence meaning structure, focusing on the Abstract Meaning Representation (AMR; Banarescu et al. 2013) parsing formalism, which provides rich graphical representations of sentence meaning structure while abstracting away from surface forms. We compare models' analysis of this semantic structure across two settings: 1) direct production of AMR parses based on zero- and few-shot prompts, and 2) indirect partial reconstruction of AMR via metalinguistic natural language queries (e.g., "Identify the primary event of this sentence, and the predicate corresponding to that event."). Across these settings, we find that models can reliably reproduce the basic format of AMR, and can often capture core event, argument, and modifier structure -- however, model outputs are prone to frequent and major errors, and holistic analysis of parse acceptability shows that even with few-shot demonstrations, models have virtually 0% success in producing fully accurate parses. Eliciting natural language responses produces similar patterns of errors. Overall, our findings indicate that these models out-of-the-box can capture aspects of semantic structure, but there remain key limitations in their ability to support fully accurate semantic analyses or parses.

==> sections/9-notes.tex <==
% \section{NOTES}


% \subsection{data selection.}
% Sort by length distribution
% Select 10

% \subsection{}

% for appendix: 
% %https://amr.isi.edu/download.html
% overlap with propbank


% \section{Valentina's notes}



==> sections/sketch.tex <==

\section{Sketch}

\ake{NOTE: this sketch is now out of date. We were considering expanding to other semantic/syntactic annotation formalisms, but we have subsequently shifted away from that scope.}
\subsection{Set-up}
LLMs have revolutionized NLP with their ability to support performance of all kinds of tasks. While this was previously enabled through fine-tuning, the most recent models have shown amazing zero- and few-shot performance (“emergent capabilities”) across diverse task types, including writing poetry, syllabi, and code, creating unusual content/style mixtures in writing, providing practical advice, etc. These impressive capabilities are conducted through the medium of language, and the ability of models to respond to complex instructions in seemingly nuanced ways is suggestive of strong competence in “language understanding”. 

In this paper we will take a closer look at the language capabilities of these models – with a focus not just on how well these models use language, but the extent to which these models encode knowledge *about* language. \val{is it about language in general or do we want to narrow it down to "meaning"/semantics/structured representations?} This matters because 1) it has important implications for the ability of these models to replace supervised models for these types of annotation tasks, and 2) the extent to which we can coax this information out of models also has implications for the extent to which models have managed to represent / gain sensitivity to this information at a humanlike level. 

We focus on the case study of semantic parsing, since the ability of models to dissect the meaning components of language has particularly core implications for language understanding. 

\subsection{Zero-shot text-to-parse prompting}
We start with zero-shot, direct text-to-parse setting. This allows us to investigate the extent to which the specialized concept of semantic parsing is already familiar to the models from pre-training. 

% \paragraph{Possible things to include}
% \begin{itemize}
%     \item Try prompting using specific terms like AMR parse, propbank maybe ... 
%     \item As we’ve discussed, try sentences both with and without parses available online
%     \item Compare GPT-3, ChatGPT, GPT-4
% \end{itemize}

\paragraph{Set of zero-shot prompts}

(Brainstorming) \ake{Here I am trying to get a sense of the number of different zero-shot tests we want to include. Whatever set of prompts we settle on, we can run tests with those 1) for all three models, and 2) with sentences that are and aren't annotated in corpora online.}\jena{2) is only for AMR prompts right?}
\begin{itemize}
    \item ``Sentence: [insert]. Provide a semantic parse for this sentence.'' \ake{formalism-agnostic version}
    \item ``Sentence: [insert]. Provide a/the AMR parse for this sentence.''
    \item ``Sentence: [insert]. Provide a/the COGS-style semantic parse for this sentence.''
    \item ``Sentence: [insert]. Provide semantic role labeling for this sentence.'' \jena{same as pb}
    \item ``Sentence: [insert]. Provide the dependency parse for this sentence.'' \jena{now i'm wondering should we do dep? What do we get out of it?}\val{it's a less shallow representation with a lot of available training data, so an interesting datapoint imo}
    \item ``Sentence: [insert]. Provide all PropBank annotations for this sentence.''
\end{itemize}

\subsection{Few-shot text-to-parse prompting}
Next we try shifting to a few-shot setting, still prompting models to generate parses directly. This moves from asking what specialized knowledge models already have about this task, to asking to what extent they can take examples of this annotation scheme and generalize to new examples using knowledge about the relevant semantic information. 

% \paragraph{Possible things to include}
% \begin{itemize}
% \item Report what we’ve found so far with AMR (limitations relative to SOTA, but improvements with similarity-based sampling, generally able to produce decent parses)
% \item Could also include some examples from simpler semantic parsing schemes (I did a small amount of testing with this early on, e.g. COGS style parses.)
% \end{itemize}

\paragraph{Set of few-shot experiments}

(Brainstorming) \ake{Here once again I'm trying to get a handle on how many experiments we would want included within the few-shot section.}
\begin{itemize}
    \item Few-shot AMR (with random and similarity-based sampling? only similarity-based?) \ake{This is what we already have, unless we want to try additional sampling schemes}
    \item Few-shot SRL (also multiple types of sampling? presumably same as whatever we decide to keep for AMR)
    \item Few-shot COGS
    \item Few-shot dependency parsing
    \item Few-shot ... PropBank annotations?
\end{itemize}

\subsection{Zero-shot NL-based prompting}
In both of the above settings, we are asking models to produce a format of output that is not natural language. Though these models have shown impressive capabilities even with less standard natural language outputs, we may get more traction from them by asking questions that prompt models to provide natural language responses that contain the kind of structural information captured in these different types of parses. This is also more parallel to the way that this kind of information can be coaxed from humans who don’t have training in this kind of linguistic analysis.

% \paragraph{Possible things to include}
% \begin{itemize}
% \item successes we are seeing with certain meta-linguistic questions
% \item mixed success with having it generate questions for itself
% \item better performance with questions about "clauses", "subject", "object" than more semantic notions like "agent", etc
% \end{itemize}

\paragraph{Set of zero-shot NL experiments (or maybe also few-shot NL)?}

(Brainstorming) \ake{If possible, would be good to divide this section similarly to the other two sections, where the NL content we are eliciting is content for AMR, for dependency parses, for SRL, etc.}
\begin{itemize}
    \item Meta-linguistic questions we have been asking to extract AMR parses.
    \item QASRL-style questions targeting lower-level SR stuff? This might serve as a parallel to the COGS/SRL from the earlier sections.
    \item Syntactic dependency questions to correspond to dependency parsing?
    \item \emph{Possible addendum: Also zero- or one-shot prompts to make models generate their own QASRL/meta-linguistic questions? Will this take us too far out in scope?} \val{might be interesting if we have enough time left}
\end{itemize}

